Quantum coherent and measurement feedback control based on atoms coupled with a semi-infinite waveguide

In this paper, we show that quantum feedback control may be applied to generate desired states for atomic and photonic systems based on a semi-infinite waveguide coupled with multiple two-level atoms. In this set-up, an initially excited atom can emit one photon into the waveguide, which can be reflected by the terminal mirror or other atoms to establish different feedback loops via the coherent interactions between the atom and photon. When there are at most two excitations in the waveguide quantum electrodynamics (waveguide QED) system, the evolution of quantum states can be interpreted using random graph theory. While this process is influenced by the environment, and we clarify that the environment-induced dynamics can be eliminated by measurement-based feedback control or coherent drives. Thus, in the open system atom-waveguide interactions, measurement-based feedback can modulate the final steady quantum state, while simultaneously, the homodyne detection noise in the measurement process can induce oscillations, which is treated by the coherent feedback designs.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
%\newsiamremark{theorem}{Theorem}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Quantum feedback, atoms and semi-infinite waveguide}{Quantum feedback, atoms, and semi-infinite waveguide}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{
Quantum coherent and measurement feedback control based on atoms coupled with a semi-infinite waveguide%\thanks{Submitted to the editors DATE.
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}
\thanks{%Submitted to the editors DATE.
%\funding{
This work is supported by the ANR project  Q-COAST ANR-19-CE48-0003  and the ANR project IGNITION ANR-21-CE47-0015.}}


\author{Haijin Ding\thanks{Laboratoire des Signaux et Syst\`{e}mes (L2S), CNRS-CentraleSup\'{e}lec-Universit\'{e} Paris-Sud, Universit\'{e} Paris-Saclay, 3, Rue Joliot Curie, 91190, Gif-sur-Yvette, France. 
  (\email{dhj17@tsinghua.org.cn})} \and Nina H. Amini\thanks{Laboratoire des Signaux et Syst\`{e}mes (L2S), CNRS-CentraleSup\'{e}lec-Universit\'{e} Paris-Sud, Universit\'{e} Paris-Saclay, 3, Rue Joliot Curie, 91190, Gif-sur-Yvette, France. 
  (\email{ nina.amini@l2s.centralesupelec.fr}).}
 \and Guofeng Zhang\thanks{Department of Applied Mathematics, The Hong Kong Polytechnic University, Hung Hom, Kowloon,  SAR, China, and The Hong Kong Polytechnic University Shenzhen Research Institute, Shenzhen, 518057, China (\email{guofeng.zhang@polyu.edu.hk}).}
 \and John E. Gough\thanks{Aberystwyth University, SY23 3BZ, Wales, United Kingdom (\email{ jug@aber.ac.uk}).}
}





% \author[1]{Haijin Ding}
% \affil[1]{Laboratoire des Signaux et Syst\`{e}mes (L2S), CNRS-CentraleSup\'{e}lec-Universit\'{e} Paris-Sud, Universit\'{e} Paris-Saclay, 3, Rue Joliot Curie, 91190, Gif-sur-Yvette, France. 
% }


\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
%%% END HELPER CODE
%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
